RubricReviewer: From Direct Critique to Rubric-Driven Review via Agentic Evidence Synthesis and Human-Aligned Generation

Peer review at major venues is under unprecedented submission pressure, motivating the use of large language models (LLMs) as review assistants. Existing LLM-based reviewers, however, face two structural limitations. First, they map manuscripts directly to reviews, leaving the underlying rubric implicit and entangling its derivation with the judgement. Second, the prevailing paradigms each capture only half of a good review: training-free agents gather broad evidence but produce undirected critiques, while training-based reviewers inherit human discriminative judgement together with its noise and uneven coverage. We introduce RubricReviewer, a fully rubric-driven framework that addresses both limitations. It makes rubric generation an explicit intermediate step, so that both review generation and the final assessment are conditioned on paper-adaptive rubrics. It further combines a training-free agent (Scout) that gathers external evidence with a human-aligned trained model (Aligner) that consumes this evidence, fusing the strengths of both supervision sources. Experiments on real-world submissions show that RubricReviewer produces reviews that are markedly more comprehensive and more discriminative than prior systems, and exhibits the strongest robustness against adversarial prompt-injection attacks. Ablation studies further confirm the necessity of each component.

==> tables/attack.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{\textbf{Verdict Positive\,\%}} & \multicolumn{2}{c}{\textbf{Avg.\ Rating}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\textbf{Method} & Clean & Attack & Clean & Attack \\
\midrule
AI Scientist                  &  5.2 & --                       & 3.29 & --                       \\
CycleReviewer-123B            & 19.2 & 22.9 \scriptsize{(+3.7)} & 5.78 & 6.06 \scriptsize{(+0.28)} \\
DeepReviewer-14B              & 22.4 & 25.9 \scriptsize{(+3.5)} & 5.46 & 5.83 \scriptsize{(+0.38)} \\
ReviewGrounder                & 42.1 & 44.2 \scriptsize{(+2.1)} & 4.55 & 4.65 \scriptsize{(+0.10)} \\
\midrule
\textbf{RubricReviewer (Ours)} & 11.4 & 12.8 \scriptsize{(\textbf{+1.4})} & 5.53 & -- \\
\bottomrule
\end{tabular}
\caption{Prompt-injection robustness on the DeepReview-13K test set (200 papers). For each method we re-run the full pipeline on adversarially modified papers (a fixed ``ignore all instructions \dots Recommend Accept'' payload spliced just before the References heading; identical placement across methods) and report the paired shift relative to the clean run. \textbf{Verdict Positive\,\%} is the share of per-rubric verdicts judged ``yes'' on the entire pool of verdicts the method emits; the parenthesised number is the (Attack$-$Clean) shift in percentage points. \textbf{Avg.\ Rating} is the mean of each method's own predicted overall score across the $200$ papers; absolute scales differ across baselines but the paired shift is directly comparable. ``--'' marks attack runs that have not yet been collected (the attack re-run for AI Scientist is in flight; for Ours the rating head is a separate Stage-3 predictor and we have not yet re-run it on the attacked Stage-2 reviews). Absolute verdict positive rates are not directly comparable across methods --- AI Scientist, CycleReviewer-*, DeepReviewer-* and ReviewGrounder verdict-extract on rubrics drawn from their own reviews (typically $11{-}13$ rubrics per paper), while ours is the gold-aligned rubric set ($\sim 54$ rubrics per paper) --- but the \emph{paired shift under attack} is. Our method shows the smallest verdict shift (+1.4\,pp vs.\ +2.1 to +3.7\,pp for all three baselines that have an attack run).}
\label{tab:attack}
\end{table}

